On the Importance of Super-Gaussian Speech Priors for Machine-Learning Based Speech Enhancement

For enhancing noisy signals, machine-learning based single-channel speech enhancement schemes exploit prior knowledge about typical speech spectral structures. To ensure a good generalization and to meet requirements in terms of computational complexity and memory consumption, certain methods restrict themselves to learning speech spectral envelopes. We refer to these approaches as machine-learning spectral envelope (MLSE)-based approaches. In this paper we show by means of theoretical and experimental analyses that for MLSE-based approaches, super-Gaussian priors allow for a reduction of noise between speech spectral harmonics which is not achievable using Gaussian estimators such as the Wiener filter. For the evaluation, we use a deep neural network (DNN)-based phoneme classifier and a low-rank nonnegative matrix factorization (NMF) framework as examples of MLSE-based approaches. A listening experiment and instrumental measures confirm that while super-Gaussian priors yield only moderate improvements for classic enhancement schemes, for MLSE-based approaches super-Gaussian priors clearly make an important difference and significantly outperform Gaussian priors.

==> colorconverter.tex <==
\usepackage{forloop}
\newcounter{colormap_cnt}%
\newcounter{filecnt}

\newcommand{\imgPath}{.}

\makeatletter
\newcommand{\getImage}[2][]{%
    \pgfkeysgetvalue{/pgfplots/colormap name}{\mycmname}%
    \pgfplotsarraysizetomacro{pgfpl@cm@\mycmname}\to\myarraysize%
    \setcounter{colormap_cnt}{0}
    \edef\mycolorstring{}%
    \forloop{colormap_cnt}{0}{\value{colormap_cnt} < \myarraysize}{%
        \pgfplotscolormapgetindex{\arabic{colormap_cnt}}{\mycmname}%
        \edef\mycolorstring{\mycolorstring \pgfmathresult;}%
    }%

    \newread\myhandle%
    \openin\myhandle=#2%
    \read\myhandle to \mytrash
    \read\myhandle to \mytrash
    \read\myhandle to \myxmin
    \read\myhandle to \myxmax
    \read\myhandle to \myymin
    \read\myhandle to \myymax
    \read\myhandle to \mydatapmin
    \read\myhandle to \mydatapmax
    \closein\myhandle%
    \pgfkeysgetvalue{/pgfplots/point meta min}{\mystylepmin}
    \ifx\empty\mystylepmin
    \edef\mypmin{\mydatapmin}
    \else
    \edef\mypmin{\mystylepmin}
    \fi
    \pgfkeysgetvalue{/pgfplots/point meta max}{\mystylepmax}
    \ifx\empty\mystylepmax
    \edef\mypmax{\mydatapmax}
    \else
    \edef\mypmax{\mystylepmax}
    \fi
    \edef\myfilecnt{\thefilecnt}

    \tikzifexternalizing{\tikzexternalgetnextfilename\filename\eappto\filename{-\myfilecnt}}{\edef\filename{\imgPath/\jobname-\myfilecnt}}

    \immediate\write18{./colorconverter.py "#2" "\mycolorstring" "\mypmin" "\mypmax" "\filename.png"}%
    \addplot[point meta min=\mypmin, point meta max=\mypmax, #1] graphics [xmin=\myxmin, xmax=\myxmax, ymin=\myymin, ymax=\myymax] {\filename.png};
    \stepcounter{filecnt}
}
\makeatother

